Analyzing Ta-Shma's Code via the Expander Mixing Lemma

Random walks in expander graphs and their various derandomizations (e.g., replacement/zigzag product) are invaluable tools from pseudorandomness. Recently, Ta-Shma used s-wide replacement walks in his breakthrough construction of a binary linear code almost matching the Gilbert-Varshamov bound (STOC 2017). Ta-Shma's original analysis was entirely linear algebraic, and subsequent developments have inherited this viewpoint. In this work, we rederive Ta-Shma's analysis from a combinatorial point of view using repeated application of the expander mixing lemma. We hope that this alternate perspective will yield a better understanding of Ta-Shma's construction. As an additional application of our techniques, we give an alternate proof of the expander hitting set lemma.

==> sections/defs2.tex <==
%%% The Protocol Box!!
\newcommand{\pprotocol}[5]{{\begin{figure}[#3]
\begin{center}
\fbox{
\hbox{\quad
\begin{minipage}{#4\textwidth}
\small
#5
\end{minipage}
\quad} }
\caption{\label{#2} #1}
\end{center}
\end{figure} } }

\newcommand{\myprotocol}[4]{\pprotocol{#1}{#2}{htp!}{#3}{#4}}
\newcommand{\numberthis}{\addtocounter{equation}{1}\tag{\theequation}}

%%%%  Authors' comments....
\newif\ifnotes
\notestrue
\ifnotes
\newcommand{\silas}[1]{ %% Silas
\vskip 1mm\noindent\hspace{.5cm}
\begin{tikzpicture}
\tikzstyle{block} = [draw, rectangle, fill=green!50, rounded corners, text width=12cm, minimum height=.85cm]
\node [block] (A) {\textbf{SILAS:} #1};
\end{tikzpicture}
\vskip 1mm\noindent\hspace{.5cm}
}

\newcommand{\sourya}[1]{ %% Sourya
\vskip 1mm\noindent\hspace{.5cm}
\begin{tikzpicture}
\tikzstyle{block} = [draw, rectangle, fill=blue!50, rounded corners, text width=12cm, minimum height=.85cm]
\node [block] (A) {\textbf{SOURYA:} #1};
\end{tikzpicture}
\vskip 1mm\noindent\hspace{.5cm}
}

\makeatletter
\newcommand{\stackalign}[1]{
  \vcenter{
    \Let@ \restore@math@cr \default@tag
    \baselineskip\fontdimen10 \scriptfont\tw@
    \advance\baselineskip\fontdimen12 \scriptfont\tw@
    \lineskip\thr@@\fontdimen8 \scriptfont\thr@@
    \lineskiplimit\lineskip
    \ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\crcr
      #1\crcr
    }
  }
}


\makeatletter
\def\legendre@dash#1#2{\hb@xt@#1{%
  \kern-#2\p@
  \cleaders\hbox{\kern.5\p@
    \vrule\@height.2\p@\@depth.2\p@\@width\p@
    \kern.5\p@}\hfil
  \kern-#2\p@
  }}
\def\@legendre#1#2#3#4#5{\mathopen{}\left(
  \sbox\z@{$\genfrac{}{}{0pt}{#1}{#3#4}{#3#5}$}%
  \dimen@=\wd\z@
  \kern-\p@\vcenter{\box0}\kern-\dimen@\vcenter{\legendre@dash\dimen@{#2}}\kern-\p@
  \right)\mathclose{}}
\newcommand\legendre[2]{\mathchoice
  {\@legendre{0}{1}{}{#1}{#2}}
  {\@legendre{1}{.5}{\vphantom{1}}{#1}{#2}}
  {\@legendre{2}{0}{\vphantom{1}}{#1}{#2}}
  {\@legendre{3}{0}{\vphantom{1}}{#1}{#2}}
}
\def\dlegendre{\@legendre{0}{1}{}}
\def\tlegendre{\@legendre{1}{0.5}{\vphantom{1}}}
\makeatother




\def\namedlabel#1#2{\begingroup
	#2%
	\def\@currentlabel{#2}%
	\phantomsection\label{#1}\endgroup
}
%%%%
%%%%  Some commands....
%%%%

%%%%%% bfs..
\newcommand{\bE}{{\bf E}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bz}{{\bf z}}
\newcommand{\bzero}{{\bf 0}}

%%%%%% math bbs..
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\I}{\mathbb{I}}
%%%%%% cals..
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calB}{\mathcal{B}}

%%%%%% sfs..
\newcommand{\p}{{\sf p}}
\newcommand{\q}{{\sf q}}
\newcommand{\rand}{{\sf rand}}
\newcommand{\rhs}{{\sf RHS}}
\newcommand{\rw}{{\sf RW}}
\newcommand{\sw}{s{\sf RW}}
\newcommand{\sfa}{{\sf a}}
\newcommand{\sfA}{{\sf A}}
\newcommand{\sfb}{{\sf b}}
\newcommand{\sfB}{{\sf B}}
\newcommand{\sfc}{{\sf c}}
\newcommand{\sfC}{{\sf C}}
\newcommand{\sfD}{{\sf D}}
\newcommand{\sfDaff}{{\sf D}_{\sf aff}}
\newcommand{\sfDltnm}{{\sf D}_{\sf LTNM}}
\newcommand{\sfE}{{\sf E}}
\newcommand{\sfEaff}{{\sf E}_{\sf aff}}
\newcommand{\sfEltnm}{{\sf E}_{\sf LTNM}}
\newcommand{\sff}{{\sf f}}
\newcommand{\sfF}{{\sf F}}
\newcommand{\sfg}{{\sf g}}
\newcommand{\sfG}{{\sf G}}
\newcommand{\sfh}{{\sf h}}
\newcommand{\sfH}{{\sf H}}
\newcommand{\sfL}{{\sf L}}
\newcommand{\sfN}{{\sf N}}
\newcommand{\sfP}{{\sf P}}
\newcommand{\sfPhi}{{\sf \Phi}}
\newcommand{\sfS}{{\sf S}}
\newcommand{\sfSIM}{{\sf SIM}}
\newcommand{\sfT}{{\sf T}}
\newcommand{\sfTltnm}{{\sf T}_{\sf LTNM}}
\newcommand{\sfV}{{\sf V}}
\newcommand{\val}{{\sf val}}
\newcommand{\sfX}{{\sf X}}
%\newcommand{\sfN}{{\sf N}}
\newcommand{\sfu}{{\sf u}}
\newcommand{\supp}{{\mathrm{supp}}}
\newcommand{\z}{{\sf z}}
%\newcommand{\cov}{{\sf{ \small COV}}}
\newcommand{\cov}{\scriptsize{\sf{  Cov}}}
\newcommand{\sfvar}{{\sf{ \small Var}}}
\newcommand{\sfv}{{\sf v}}
%%%%%% overlines..
\newcommand{\overa}{\overline{\sf a}}
\newcommand{\overA}{\overline{\sf A}}
\newcommand{\overb}{\overline{\sf b}}
\newcommand{\overB}{\overline{\sf B}}
\newcommand{\overc}{\overline{\sf c}}
\newcommand{\overC}{\overline{\sf C}}

%%%%%% others..
\newcommand{\boldone}{{1\!\!1}}
\newcommand{\dec}{{\sf Dec}}
\newcommand{\dist}{{\sf dist}}
\newcommand{\enc}{{\sf Enc}}
\newcommand{\ep}{\varepsilon}
\newcommand{\niceand}{\text{ }\&\text{ }}
\newcommand{\niceforall}{\text{ }\forall\text{ }}
\newcommand{\poly}{{\sf poly}}
\newcommand{\prob}[1]{{\rm Pr}_{#1}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\test}{{\sf Test}}

\newcommand{\bv}{{\boldsymbol{v}}}



%%%Agreements
\newcommand{\apa}{{\mathcal{A}_{\tilde\alpha\tilde\Phi\tilde\alpha'}}}
\newcommand{\bpb}{{\mathcal{A}_{\tilde\beta\tilde\Phi\tilde\beta'}}}
\newcommand{\gpg}{{\mathcal{A}_{\tilde\gamma\tilde\Phi\tilde\gamma'}}}
\newcommand{\aga}{{\mathcal{A}_{\tilde\alpha\tilde\gamma\tilde\alpha'}}}
\newcommand{\agsa}{{\mathcal{A}_{\tilde\alpha\tilde\gamma^*\tilde\alpha'}}}
\newcommand{\pg}{{\mathcal{A}_{\tilde\Phi\tilde\gamma}}}
\newcommand{\ag}{{\mathcal{A}_{\tilde\alpha\tilde\gamma}}}
\newcommand{\abgs}{{\mathcal{A}_{\tilde\alpha\tilde\beta\tilde\gamma^*}}}
\newcommand{\abg}{{\mathcal{A}_{\tilde\alpha\tilde\beta\tilde\gamma'}}}
\newcommand{\gag}{{\mathcal{A}_{\tilde\gamma\tilde\alpha\tilde\gamma'}}}
\newcommand{\abgd}{{\mathcal{A}_{\tilde\alpha\tilde\beta\tilde\gamma''}}}
\newcommand{\gagd}{{\mathcal{A}_{\tilde\gamma\tilde\alpha\tilde\gamma''}}}
\newcommand{\gpgd}{{\mathcal{A}_{\tilde\gamma\tilde\Phi\tilde\gamma''}}}

\newcommand{\ap}{{\mathcal{A}_{\tilde\alpha\tilde\Phi}}}

\newcommand{\app}{{\mathcal{A}_{\tilde\alpha'\tilde\Phi'}}}

\newcommand{\appp}{{\mathcal{A}_{\tilde\alpha''\tilde\Phi''}}}

\newcommand{\gapp}{{\mathcal{A}_{\tilde\gamma'\tilde\alpha'\tilde\Phi'}}}

%%%%  Some Theorems....
\newtheorem{clm}{Claim}
\newtheorem{defn}{Definition}
\newtheorem{thm}{Theorem}
\newtheorem{fact}{Fact}
